Lagrangian PINNs: A causality-conforming solution to failure modes of physics-informed neural networks

Physics-informed neural networks (PINNs) leverage neural-networks to find the solutions of partial differential equation (PDE)-constrained optimization problems with initial conditions and boundary conditions as soft constraints. These soft constraints are often considered to be the sources of the complexity in the training phase of PINNs. Here, we demonstrate that the challenge of training (i) persists even when the boundary conditions are strictly enforced, and (ii) is closely related to the Kolmogorov n-width associated with problems demonstrating transport, convection, traveling waves, or moving fronts. Given this realization, we describe the mechanism underlying the training schemes such as those used in eXtended PINNs (XPINN), curriculum regularization, and sequence-to-sequence learning. For an important category of PDEs, i.e., governed by non-linear convection-diffusion equation, we propose reformulating PINNs on a Lagrangian frame of reference, i.e., LPINNs, as a PDE-informed solution. A parallel architecture with two branches is proposed. One branch solves for the state variables on the characteristics, and the second branch solves for the low-dimensional characteristics curves. The proposed architecture conforms to the causality innate to the convection, and leverages the direction of travel of the information in the domain. Finally, we demonstrate that the loss landscapes of LPINNs are less sensitive to the so-called "complexity" of the problems, compared to those in the traditional PINNs in the Eulerian framework.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Lagrangian PINN}{R. Mojgani, M. Balajewicz, and P. Hassanzadeh}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Lagrangian PINNs: \\
	A causality--conforming solution to failure modes\\
	of physics-informed neural networks
	\thanks{\color{\mycolor}Submitted to the editors May 4, 2022.
	\funding{\color{\mycolor}
		This work was supported by an award from the ONR Young Investigator Program (N00014-20-1-2722), a grant from the NSF CSSI program (OAC-2005123), and by the generosity of Eric and Wendy Schmidt by recommendation of the Schmidt Futures program. Computational resources
		were provided by NSF XSEDE (allocation ATM170020) and NCAR's CISL (allocation URIC0004).
	Our codes and data are available at~\mydepository.}
}}

% Authors: full names plus addresses.
\author{
	Rambod Mojgani\thanks{Rice University, Houston, TX 
		   (\email{rm99@rice.edu}).}%, \url{http://www.imag.com/}).}
\and Maciej Balajewicz\thanks{Realtor.com, Santa Clara, CA}
\and Pedram Hassanzadeh\thanks{Rice University, Houston, TX}
}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

